Unraveling the Smoothness Properties of Diffusion Models: A Gaussian Mixture Perspective

Diffusion models have made rapid progress in generating high-quality samples across various domains. However, a theoretical understanding of the Lipschitz continuity and second momentum properties of the diffusion process is still lacking. In this paper, we bridge this gap by providing a detailed examination of these smoothness properties for the case where the target data distribution is a mixture of Gaussians, which serves as a universal approximator for smooth densities such as image data. We prove that if the target distribution is a $k$-mixture of Gaussians, the density of the entire diffusion process will also be a $k$-mixture of Gaussians. We then derive tight upper bounds on the Lipschitz constant and second momentum that are independent of the number of mixture components $k$. Finally, we apply our analysis to various diffusion solvers, both SDE and ODE based, to establish concrete error guarantees in terms of the total variation distance and KL divergence between the target and learned distributions. Our results provide deeper theoretical insights into the dynamics of the diffusion process under common data distributions.

==> 14_app_softmax.tex <==
\section{Tools Related Softmax}

In Section~\ref{sec:preliminary:definitions} provides the definitions of softmax score function.

\subsection{Definitions}\label{sec:preliminary:definitions}
\begin{definition}\label{def:alpha_no_t}
If the following conditions hold
\begin{itemize}
    \item Let us consider the discrete setting, where $x_1, x_2, \cdots, x_n$.
    \item  Let $X= [x_1 ~ x_2 ~ \cdots ~ x_n]^\top \in \R^{n \times d}$.
    \item Let $a \in \R^d$.
\end{itemize}

We define
\begin{align*}
    \underbrace{\alpha(X)}_{\mathrm{scalar}} := \underbrace{\langle {\bf 1}_n , \exp(X a ) \rangle}_{\mathrm{scalar}}
\end{align*}
\end{definition}

The softmax pmf for discrete case when there is no time considered.

\begin{definition}\label{def:p_t_no_t}
If the following conditions hold
\begin{itemize}
    \item Let us consider the discrete setting, where $x_1, x_2, \cdots, x_n$.
    \item  Let $X= [x_1 ~ x_2 ~ \cdots ~ x_n]^\top \in \R^{n \times d}$.
    \item Let $a \in \R^d$.
\end{itemize}
 
We define 
\begin{align*}
    \underbrace{p_t(x_i)}_{\mathrm{scalar}} := \underbrace{\langle {\bf 1}_n, \exp(X a) \rangle^{-1}}_{\mathrm{scalar}} \underbrace{\exp(\langle x_i, a\rangle)}_{\mathrm{scalar}}
\end{align*}

Further, we can rewrite $p_t(x_i)$ as follows:
\begin{align*}
    \underbrace{p_t(x_i)}_{\mathrm{scalar}} = \underbrace{\alpha(X)^{-1}}_{\mathrm{scalar}} \underbrace{\exp( \langle x_i, a\rangle )}_{\mathrm{scalar}}
\end{align*}
\end{definition}


 
\begin{lemma}\label{lem:gradient_inner_xa}
If the following conditions hold
\begin{itemize}
    \item Let $x_i \in \R^d$ for $i=1,2,\dots,n$. 
    \item Let $a \in \R^d$.
\end{itemize}

Then for each $i \in [n], j \in [d]$
\begin{align*}
    \underbrace{\frac{\d \langle x_i, a \rangle}{\d x_{i,j}}}_{\mathrm{scalar}} = \underbrace{a_j}_{\mathrm{scalar}}
\end{align*}
\end{lemma}

\begin{proof}
We can show
\begin{align*}
    \frac{\d \langle x_i, a \rangle}{\d x_{i,j}} = & ~ \frac{\d \sum_{j=1}^d x_{i,j} a_j}{\d x_{i,j}}\\
    = & ~ \frac{\d x_{i,j} a_j}{\d x_{i,j}}\\
    = & ~ a_j
\end{align*}    
where the first step follows from the notation of the inner product, the second step follows from Fact~\ref{fac:calculus}, and the last step follows from Fact~\ref{fac:calculus}.
\end{proof}

\begin{lemma}\label{lem:gradient_Xa}
If the following conditions hold 
\begin{itemize}
    \item Let $x_i \in \R^d$ for $i=1,2,\dots,n$. 
    \item Let $a \in \R^d$.
    \item Let $X= [x_1 ~ x_2 ~ \cdots ~ x_n]^\top \in \R^{n \times d}$.
\end{itemize}
Then, for each $i \in [n]$, $j \in [d]$, we have
\begin{align*}
    \underbrace{ \frac{\d Xa}{\d x_{i,j}} }_{n \times 1} = \underbrace{ a_j }_{\mathrm{scalar}} \cdot \underbrace{ e_i }_{n \times 1}
\end{align*}

\end{lemma}

\begin{proof}
We can show
\begin{align*}
    \underbrace{ \frac{\d Xa}{\d x_{i,j}} }_{n \times 1} = & ~ \underbrace{ \frac{\d (Xa)_i }{\d x_{i,j}} }_{ \mathrm{scalar} } \cdot \underbrace{ e_i }_{n \times 1} \\
    = & ~ \underbrace{\frac{ \d \langle x_i ,  a \rangle }{ \d x_{i,j} }}_{\mathrm{scalar}} \cdot \underbrace{e_i}_{n \times 1} \\
    = & ~ \underbrace{ a_j }_{ \mathrm{scalar} } \cdot \underbrace{ e_i }_{n \times 1} 
\end{align*}
where the first step follows from Fact~\ref{fac:calculus}, the second step follows from Fact~\ref{fac:calculus}, and the last step follows from Lemma~\ref{lem:gradient_inner_xa}.
\end{proof}


\begin{lemma}\label{lem:gradient_exp_xa}
If the following conditions hold
\begin{itemize}
    \item Let $x_i \in \R^d$ for $i=1,2,\dots,n$. 
    \item Let $a \in \R^d$.
\end{itemize}
Then, for each $i \in [n]$, we have
\begin{itemize}
\item Part 1. For each $j \in [d]$
\begin{align*}
    \underbrace{ \frac{\d \exp(\langle x_i, a \rangle ) }{ \d x_{i,j} } }_{ \mathrm{scalar} } = \underbrace{ \exp(\langle x_i, a \rangle) }_{ \mathrm{scalar} } \underbrace{ a_j }_{ \mathrm{scalar} }
\end{align*}
\item Part 2. For each $i$
\begin{align*}
    \underbrace{ \frac{\d \exp(\langle x_i, a \rangle ) }{ \d x_{i} } }_{d \times 1} =  \underbrace{ \exp(\langle x_i, a \rangle) }_{ \mathrm{scalar} } \underbrace{ a }_{d \times 1}
\end{align*}
\item Part 3. For each $k \neq i$, $j \in [d]$
\begin{align*}
    \underbrace{\frac{ \d \exp(\langle x_i, a \rangle) }{ \d x_{k,j} }}_{\mathrm{scalar}} = 0
\end{align*}
\end{itemize}
\end{lemma}

\begin{proof}
Now we prove for each part:

{\bf Proof of Part 1.}
\begin{align*}
    \frac{\d \exp(\langle x_i, a \rangle ) }{ \d x_{i,j} } = & ~ \frac{\d \exp(\langle x_i, a \rangle ) }{ \d \langle x_i, a\rangle } \frac{\d \langle x_i, a\rangle}{\d x_{i,j}}\\
    = & ~ \exp(\langle x_i, a \rangle) \frac{\d \langle x_i, a\rangle}{\d x_{i,j}}\\
    = & ~ \exp(\langle x_i, a \rangle) a_j
\end{align*}
where the first step follows from Fact~\ref{fac:calculus}, the second step follows from Fact~\ref{fac:calculus}, and the last step follows from Lemma~\ref{lem:gradient_inner_xa}.

{\bf Proof of Part 2.}
\begin{align*}
    \frac{\d \exp(\langle x_i, a \rangle ) }{ \d x_{i} } = & ~ \frac{\d \exp(\langle x_i, a \rangle ) }{ \d \langle x_i, a\rangle } \frac{\d \langle x_i, a\rangle}{\d x_{i}}\\
    = & ~ \exp(\langle x_i, a \rangle) \frac{\d \langle x_i, a\rangle}{\d x_{i}}\\
    = & ~ \exp(\langle x_i, a \rangle) a
\end{align*}
where the first step follows from Fact~\ref{fac:calculus}, the second step follows from Fact~\ref{fac:calculus}, and the last step follows from Fact~\ref{fac:calculus}.

{\bf Proof of Part 3.}
For each $k \neq i$
\begin{align*}
    \frac{\d \exp(\langle x_i, a \rangle ) }{ \d x_{k,j} } = & ~ \frac{\d \exp(\langle x_i, a \rangle ) }{ \d \langle x_i, a\rangle } \frac{\d \langle x_i, a\rangle}{\d x_{k,j}}\\
    = & ~ \frac{\d \exp(\langle x_i, a \rangle ) }{ \d \langle x_i, a\rangle } \cdot 0\\
    = & ~ 0
\end{align*}
where the first step follows from Fact~\ref{fac:calculus}, the second step follows from variables are independent, and the last step follows from simple algebra.

\end{proof}

\begin{lemma}
If the following conditions hold
\begin{itemize}
    \item Let $x_i \in \R^d$ for $i=1,2,\dots,n$. 
    \item Let $a \in \R^d$.
    \item Let $X= [x_1 ~ x_2 ~ \cdots ~ x_n]^\top \in \R^{n \times d}$.
\end{itemize}
Then we can show, for each $i \in [n]$, $j\in [d]$
\begin{itemize}
    \item
    \begin{align*}
        \underbrace{\frac{\d \exp(Xa)}{ \d x_{i,j} }}_{n \times 1} = \underbrace{e_i}_{n \times 1} \circ \underbrace{ \exp(Xa) }_{n \times 1} \underbrace{ a_j }_{ \mathrm{scalar} }
    \end{align*}
\end{itemize}
\end{lemma}

\begin{proof}
We know that $\underbrace{ \exp(Xa) }_{n \times 1}$ and $\underbrace{ x_{i,j} }_{ \mathrm{scalar}}$, so the result must also be an $\R^n$ vector.

Then, we can show
\begin{align*}
    \underbrace{\frac{\d \exp(Xa)}{ \d x_{i,j} }}_{n \times 1} = & ~ \underbrace{ \frac{\d \exp(Xa)_i }{\d x_{i,j}} }_{ \mathrm{scalar} } \cdot \underbrace{ e_i }_{n \times 1} \\
    = & ~ \underbrace{\frac{ \d \exp(\langle x_i ,  a \rangle)}{ \d x_{i,j}}}_{\mathrm{scalar}} \cdot \underbrace{e_i}_{n \times 1} \\
    = & ~ \underbrace{\exp(\langle x_i, a \rangle) a_j}_{\mathrm{scalar}} \cdot \underbrace{e_i}_{n \times 1}\\
    = & ~ \underbrace{ e_i \circ \exp(Xa) }_{n \times 1} \underbrace{ a_j }_{ \mathrm{scalar} }
\end{align*}
where the first step follows from Fact~\ref{fac:calculus}, the second step follows from Fact~\ref{fac:calculus}, the third step follows from Lemma~\ref{lem:gradient_exp_xa}, and the last step follows from the notation of Hardamard product.
\end{proof}

\begin{lemma}\label{lem:gradient_alpha_no_t}
If the following conditions hold
\begin{itemize}
    \item Let $\alpha(X)$ be defined as Definition~\ref{def:alpha_no_t}.
    \item Let $x_i \in \R^d$ for $i=1,2,\dots,n$. 
    \item Let $a \in \R^d$.
    \item Let $X= [x_1 ~ x_2 ~ \cdots ~ x_n]^\top \in \R^{n \times d}$.
\end{itemize}
Then, for each $i \in [n]$, we have
\begin{itemize}
\item Part 1. For each $j \in [d]$
\begin{align*}
    \underbrace{\frac{ \d \alpha(X) }{ \d x_{i,j} }}_{\mathrm{scalar}} =  \underbrace{\exp(\langle x_i, a \rangle)}_{\mathrm{scalar}} \underbrace{a_j}_{\mathrm{scalar}}
\end{align*}
\item Part 2. 
\begin{align*}
    \underbrace{\frac{ \d \alpha(X) }{ \d x_{i} }}_{d \times 1} = \underbrace{\exp(\langle x_i, a \rangle)}_{\mathrm{scalar}} \underbrace{a}_{d \times 1}
\end{align*}
\end{itemize}
\end{lemma}



\begin{proof}
We know that $\underbrace{\alpha(X)}_{ \mathrm{scalar}}$.

Now we prove for each part:

{\bf Proof of Part 1.}
\begin{align*}
    \frac{ \d \alpha(X) }{ \d x_{i,j} } = & ~ \frac{ \d  }{ \d x_{i,j} } \langle {\bf 1}_n, \exp(X a) \rangle\\
    = & ~ \frac{ \d  }{ \d x_{i,j} } \sum_{k=1}^n \exp(\langle x_k, a \rangle)\\
    = & ~ \frac{ \d  }{ \d x_{i,j} }  \exp(\langle x_i, a \rangle)\\
    = & ~ \exp(\langle x_i, a \rangle) a_j
\end{align*}
where the first step follows from the Definition~\ref{def:alpha_no_t}, the second step follows from Fact~\ref{fac:calculus}, the third step follows from Lemma~\ref{lem:gradient_exp_xa}, and the last step follows from Lemma~\ref{lem:gradient_exp_xa}.

{\bf Proof of Part 2.}
\begin{align*}
    \frac{ \d \alpha(X) }{ \d x_{i} } = & ~ \frac{ \d  }{ \d x_{i} } \langle {\bf 1}_n, \exp(X a) \rangle\\
    = & ~ \frac{ \d  }{ \d x_{i} } \sum_{k=1}^n \exp(\langle x_k, a \rangle)\\
    = & ~ \frac{ \d  }{ \d x_{i} }  \exp(\langle x_i, a \rangle)\\
    = & ~ \exp(\langle x_i, a \rangle) a
\end{align*}
where the first step follows from the Definition~\ref{def:alpha_no_t}, the second step follows from Fact~\ref{fac:calculus}, the third step follows from Lemma~\ref{lem:gradient_exp_xa}, and the last step follows from Lemma~\ref{lem:gradient_exp_xa}.
\end{proof}


\begin{lemma}\label{lem:gradient_alpha_no_t_to_neg_1}
If the following conditions hold
\begin{itemize}
    \item Let $\alpha(X)$ be defined as Definition~\ref{def:alpha_no_t}.
    \item Let $x_i \in \R^d$ for $i=1,2,\dots,n$. 
    \item Let $a \in \R^d$.
    \item Let $X= [x_1 ~ x_2 ~ \cdots ~ x_n]^\top \in \R^{n \times d}$.
\end{itemize}
Then, for each $i \in [n]$, we have
\begin{itemize}
\item Part 1. For each $j \in [d]$
\begin{align*}
    \underbrace{\frac{ \d \alpha(X)^{-1} }{ \d x_{i,j} }}_{\mathrm{scalar}} = \underbrace{- \alpha(X)^{-2}}_{\mathrm{scalar}} \underbrace{\exp(\langle x_i, a \rangle)}_{\mathrm{scalar}}  \underbrace{a_j}_{\mathrm{scalar}} 
\end{align*}
\item Part 2. 
\begin{align*}
    \underbrace{\frac{ \d \alpha(X)^{-1} }{ \d x_{i} }}_{d \times 1}  = \underbrace{- \alpha(X)^{-2}}_{\mathrm{scalar}}  \underbrace{\exp(\langle x_i, a \rangle)}_{\mathrm{scalar}}  \underbrace{a}_{d \times 1} 
\end{align*}
\end{itemize}
\end{lemma}
\begin{proof}
Now we prove for each part:

{\bf Proof of Part 1.}
\begin{align*}
    \frac{ \d \alpha(X)^{-1} }{ \d x_{i,j} } = & ~ \frac{\d \alpha(X)^{-1}}{\d \alpha(X)} \frac{\d \alpha(X)}{\d x_{i,j}}\\
    = & ~ - \alpha(X)^{-2} \frac{\d \alpha(X)}{\d x_{i,j}}\\
    = & ~ - \alpha(X)^{-2} \exp(\langle x_i, a \rangle) a_j
\end{align*}
where the first step follows from Fact~\ref{fac:calculus}, the second step follows from Fact~\ref{fac:calculus}, and the last step follows from Lemma~\ref{lem:gradient_alpha_no_t}.
    
{\bf Proof of Part 2.}
\begin{align*}
    \frac{ \d \alpha(X)^{-1} }{ \d x_{i} } = & ~ \frac{\d \alpha(X)^{-1}}{\d \alpha(X)} \frac{\d \alpha(X)}{\d x_{i}}\\
    = & ~ - \alpha(X)^{-2} \frac{\d \alpha(X)}{\d x_{i}}\\
    = & ~ - \alpha(X)^{-2} \exp(\langle x_i, a \rangle) a
\end{align*}
where the first step follows from Fact~\ref{fac:calculus}, the second step follows from Fact~\ref{fac:calculus}, and the last step follows from Lemma~\ref{lem:gradient_alpha_no_t}.

\end{proof}


\begin{lemma}\label{lem:gradient_alpha_no_t_to_neg_q}
If the following conditions hold
\begin{itemize}
    \item Let $\alpha(X)$ be defined as Definition~\ref{def:alpha_no_t}.
    \item Let $q \geq 2$ integers.
    \item Let $x_i \in \R^d$ for $i=1,2,\dots,n$. 
    \item Let $a \in \R^d$.
    \item Let $X= [x_1 ~ x_2 ~ \cdots ~ x_n]^\top \in \R^{n \times d}$.
\end{itemize}
Then, for each $i \in [n]$, we have
\begin{itemize}
\item Part 1. For each $j \in [d]$
\begin{align*}
    \underbrace{\frac{ \d \alpha(X)^{-q} }{ \d x_{i,j} }}_{\mathrm{scalar}}  = \underbrace{-q \alpha(X)^{-q-1}}_{\mathrm{scalar}}  \underbrace{\exp(\langle x_i, a \rangle)}_{\mathrm{scalar}}  \underbrace{a_j}_{\mathrm{scalar}}
\end{align*}
\item Part 2. 
\begin{align*}
    \underbrace{\frac{ \d \alpha(X)^{-q} }{ \d x_{i} }}_{d \times 1}  = \underbrace{-q \alpha(X)^{-q-1}}_{\mathrm{scalar}} \underbrace{\exp(\langle x_i, a \rangle)}_{\mathrm{scalar}}  \underbrace{a}_{d \times 1} 
\end{align*}
\end{itemize}
\end{lemma}
\begin{proof}
Now we prove for each part:

{\bf Proof of Part 1.}
\begin{align*}
    \frac{ \d \alpha(X)^{-q} }{ \d x_{i,j} } = & ~ \frac{\d \alpha(X)^{-q}}{\d \alpha(X)} \frac{\d \alpha(X)}{\d x_{i,j}}\\
    = & ~ -q \alpha(X)^{-q-1} \frac{\d \alpha(X)}{\d x_{i,j}}\\
    = & ~ -q \alpha(X)^{-q-1} \exp(\langle x_i, a \rangle) a_j
\end{align*}
where the first step follows from Fact~\ref{fac:calculus}, the second step follows from Fact~\ref{fac:calculus} and the last step follows from Lemma~\ref{lem:gradient_alpha_no_t}.
    
{\bf Proof of Part 2.}
\begin{align*}
    \frac{ \d \alpha(X)^{-q} }{ \d x_{i} } = & ~ \frac{\d \alpha(X)^{-q}}{\d \alpha(X)} \frac{\d \alpha(X)}{\d x_{i}}\\
    = & ~ -q \alpha(X)^{-q-1} \frac{\d \alpha(X)}{\d x_{i}}\\
    = & ~ -q \alpha(X)^{-q-1} \exp(\langle x_i, a \rangle) a
\end{align*}
where the first step follows from Fact~\ref{fac:calculus}, the second step follows from Fact~\ref{fac:calculus} and the last step follows from Lemma~\ref{lem:gradient_alpha_no_t}.

\end{proof}

\begin{lemma}\label{lem:gradient_p_t_no_t}
If the following conditions hold
\begin{itemize}
    \item Let $p_t(x_i)$ be defined as Definition~\ref{def:p_t_no_t}.
    \item Let $\alpha(X)$ be defined as Definition~\ref{def:alpha_no_t}.
    \item Let $x_i \in \R^d$ for $i=1,2,\dots,n$. 
    \item Let $a \in \R^d$.
    \item Let $X= [x_1 ~ x_2 ~ \cdots ~ x_n]^\top \in \R^{n \times d}$.
\end{itemize}
Then, for each $i \in [n]$, we have 
\begin{itemize}
\item Part 1. For $j\in [d]$ 
\begin{align*}
    \underbrace{\frac{\d p_t(x_i) }{ \d x_{i,j}}}_{\mathrm{scalar}} = \underbrace{- (p_t(x_i))^2 }_{\mathrm{scalar}}  \underbrace{a_j}_\mathrm{scalar}+ \underbrace{p_t(x_i)}_{\mathrm{scalar}} \underbrace{a_j}_\mathrm{scalar}
\end{align*}
\item  Part 2.
\begin{align*}
    \underbrace{\frac{\d p_t(x_i) }{ \d x_{i}}}_{d \times 1} = \underbrace{-(p_t(x_i))^2}_{\mathrm{scalar}} \underbrace{a}_{d \times 1}  + \underbrace{p_t(x_i)}_{\mathrm{scalar}} \underbrace{a}_{d \times 1}
\end{align*}
\end{itemize}
\end{lemma}

\begin{proof}
Now we prove for each part:


{\bf Proof of Part 1.}
\begin{align*}
    \frac{\d p_t(x_i) }{ \d x_{i,j}} = & ~ \frac{\d}{\d x_{i,j}} (\alpha(X)^{-1} \exp(\langle x_i, a\rangle))\\
    = & ~ (\frac{\d}{\d x_{i,j}} \alpha(X)^{-1}) \exp(\langle x_i, a\rangle) + \alpha(X)^{-1}\frac{\d}{\d x_{i,j}} \exp(\langle x_i, a\rangle)\\
    = & ~ (- \alpha(X)^{-2} \exp(\langle x_i, a \rangle) a_j) \exp(\langle x_i, a\rangle) + \alpha(X)^{-1}\frac{\d}{\d x_{i,j}} \exp(\langle x_i, a\rangle)\\
    = & ~ (- \alpha(X)^{-2} \exp(\langle x_i, a \rangle) a_j) \exp(\langle x_i, a\rangle) + \alpha(X)^{-1} \exp(\langle x_i, a \rangle) a_j\\
    = & ~ - (p_t(x_i))^2 a_j  + p_t(x_i) a_j
\end{align*}
where the first step follows from Definition~\ref{def:p_t_no_t}, the second step follows from Fact~\ref{fac:calculus}, the third step follows from Lemma~\ref{lem:gradient_alpha_no_t_to_neg_1}, the fourth step follows from Lemma~\ref{lem:gradient_exp_xa}, and the last step follows from Definition~\ref{def:p_t_no_t}.

{\bf Proof of Part 2.}
\begin{align*}
    \frac{\d p_t(x_i) }{ \d x_{i}} = & ~ \frac{\d}{\d x_{i}} (\alpha(X)^{-1} \exp(\langle x_i, a\rangle))\\
    = & ~ (\frac{\d}{\d x_{i}} \alpha(X)^{-1}) \exp(\langle x_i, a\rangle) + \alpha(X)^{-1}\frac{\d}{\d x_{i}} \exp(\langle x_i, a\rangle)\\
    = & ~ (- \alpha(X)^{-2} \exp(\langle x_i, a \rangle) a) \exp(\langle x_i, a\rangle) + \alpha(X)^{-1}\frac{\d}{\d x_{i}} \exp(\langle x_i, a\rangle)\\
    = & ~ (- \alpha(X)^{-2} \exp(\langle x_i, a \rangle) a) \exp(\langle x_i, a\rangle) + \alpha(X)^{-1} \exp(\langle x_i, a \rangle) a\\
    = & ~ - (p_t(x_i))^2 a  + p_t(x_i) a
\end{align*}
where the first step follows from Definition~\ref{def:p_t_no_t}, the second step follows from Fact~\ref{fac:calculus}, the third step follows from Lemma~\ref{lem:gradient_alpha_no_t_to_neg_1}, the fourth step follows from Lemma~\ref{lem:gradient_exp_xa}, and the last step follows from Definition~\ref{def:p_t_no_t}.
\end{proof}

The score function of softmax pmf for discrete case when there is no time considered.
\begin{lemma}
If the following conditions hold
\begin{itemize}
    \item Let $p_t(x_i)$ be defined as Definition~\ref{def:p_t_no_t}.
    \item Let $x_i \in \R^d$ for $i=1,2,\dots,n$. 
    \item Let $a \in \R^d$.
    \item Let $X= [x_1 ~ x_2 ~ \cdots ~ x_n]^\top \in \R^{n \times d}$.
\end{itemize}
Then, for each $i \in [n]$, we have
\begin{align*}
    \frac{\d \log p_t(x_i)}{\d x_i} = (1-p_t(x_i)) \cdot a 
\end{align*}
\end{lemma}

\begin{proof}
We can show
\begin{align*}
    \frac{\d \log p_t(x_i)}{\d x_i} = & ~ \frac{\d \log p_t(x_i)}{\d p_t(x_i)} \frac{\d p_t(x_i)}{\d x_i}\\
    = & ~ \frac{1}{p_t(x_i)} \frac{\d p_t(x_i)}{\d x_i}\\
    = & ~ \frac{1}{p_t(x_i)} ( - (p_t(x_i))^2 a  + p_t(x_i) a)\\
    = & ~ (1-p_t(x_i)) \cdot a
\end{align*}
where the first step follows from Fact~\ref{fac:calculus}, the second step follows from Fact~\ref{fac:calculus}, the third step follows from Lemma~\ref{lem:gradient_p_t_no_t}, and the last step follows from rearranging terms.
\end{proof}


==> 15_app_time.tex <==
\section{Time: Linear Combination}\label{sec:time_discrete}

In this section we consider the discrete case of input, and $p_t(z_i)$ to be the probability mass function (pmf) of input $z_i$, which is the linear combination of the data and Gaussian noise with time. Our goal is to compute both upper bound and Lipschitz constant for the score function i.e. the gradient of log pmf $\frac{\d \log p_t(z_i)}{\d z_i}$.

\subsection{Definitions}
\begin{definition}\label{def:z_i}
We use $z_i(t)$ to denote input data which is a linear combination of $x_i$ and $v_i$. Here $x_i$ is sampled image distribution, and $v_i$ is sampled from noise distribution ${\cal N}(0, \Sigma)$.

We define
\begin{align*}
    z_i(t) = (1 - \frac{ t} {T} ) \cdot \underbrace{ x_i }_{ \mathrm{image} } + \frac{t}{T} \underbrace{ v_i }_{ \mathrm{noise}}
\end{align*}
\end{definition}

\begin{definition}\label{def:alpha}
If the following conditions hold
\begin{itemize}
    \item Let us consider the discrete setting, where $z_1, z_2, \cdots, z_n$.
    \item  Let $Z = [z_1 ~ z_2 ~ \cdots ~ z_n]^\top \in \R^{n \times d}$.
    \item Let $a \in \R^d$.
\end{itemize}

We define
\begin{align*}
    \underbrace{\alpha(Z)}_{\mathrm{scalar}} := \underbrace{\langle {\bf 1}_n , \exp(Z a ) \rangle}_{\mathrm{scalar}}
\end{align*}
\end{definition}

The softmax pmf for discrete case when time considered.

\begin{definition}\label{def:p_t}
If the following conditions hold
\begin{itemize}
    \item Let us consider the discrete setting, where $z_1, z_2, \cdots, z_n$.
    \item  Let $Z= [z_1 ~ z_2 ~ \cdots ~ z_n]^\top \in \R^{n \times d}$.
    \item Let $a \in \R^d$.
\end{itemize}

We define 
\begin{align*}
    \underbrace{p_t(z_i)}_{\mathrm{scalar}} := \underbrace{\langle {\bf 1}_n, \exp(Z a) \rangle^{-1}}_{\mathrm{scalar}} \underbrace{\exp(\langle z_i, a\rangle)}_{\mathrm{scalar}}
\end{align*}

Further, we can rewrite $p_t(z_i)$ as follows:
\begin{align*}
    \underbrace{p_t(z_i)}_{\mathrm{scalar}} = \underbrace{\alpha(Z)^{-1}}_{\mathrm{scalar}} \underbrace{\exp( \langle z_i, a\rangle )}_{\mathrm{scalar}}
\end{align*}
\end{definition}

\subsection{Lemmas for calculation of the score function}

\begin{lemma}\label{lem:gradient_z_i}
If the following conditions hold
\begin{itemize}
    \item Let $x_i \in \R^d$ for $i=1,2,\dots,n$. 
    \item Let $z_i$ be defined as Definition~\ref{def:z_i}.
    \item Let $a \in \R^d$.
    \item Let $t \in \R$, $T \in \R$, and $0\leq t \leq T$.
\end{itemize}

Then, for each $i \in [n]$, we have
\begin{align*}
    \frac{\d z_i}{\d x_i} = 1 - \frac{ t} {T} 
\end{align*}
\end{lemma}

\begin{proof}
We can show
\begin{align*}
    \frac{\d z_i}{\d x_i} = & ~ \frac{\d }{\d x_i} ((1 - \frac{ t} {T} ) \cdot x_i + \frac{t}{T} v_i)\\
    = & ~ \frac{\d }{\d x_i} ((1 - \frac{ t} {T} ) \cdot x_i) + \frac{\d }{\d x_i} (\frac{t}{T} v_i)\\
    = & ~ \frac{\d }{\d x_i} ((1 - \frac{ t} {T} ) \cdot x_i)\\
    = & ~ 1 - \frac{ t} {T} 
\end{align*}
where the first step follows from Definition~\ref{def:z_i}, the second step follows from Fact~\ref{fac:calculus}, the third step follows from variables are independent, and the last step follows from Fact~\ref{fac:calculus}.
\end{proof}

\begin{lemma}\label{lem:gradient_inner_za}
If the following conditions hold
\begin{itemize}
    \item Let $x_i \in \R^d$ for $i=1,2,\dots,n$. 
    \item Let $z_i$ be defined as Definition~\ref{def:z_i}.
    \item Let $a \in \R^d$.
    \item Let $t \in \R$, $T \in \R$, and $0\leq t \leq T$.
\end{itemize}

Then for each $i \in [n]$
\begin{align*}
    \frac{\d \langle z_i, a \rangle}{\d x_{i}} = (1 - \frac{t}{T}) \cdot a
\end{align*}
\end{lemma}

\begin{proof}
We can show
\begin{align*}
    \frac{\d \langle z_i, a \rangle}{\d x_{i}} = & ~ \frac{\d }{\d x_{i}} \langle (1 - \frac{t}{T}) \cdot x_i + \frac{t}{T} v_i, a \rangle\\
    = & ~ \frac{\d }{\d x_{i}} (\langle (1 - \frac{t}{T}) \cdot x_i, a \rangle + \langle \frac{t}{T} v_i, a \rangle)\\
    = & ~ (1 - \frac{t}{T}) \cdot \frac{\d }{\d x_{i}} \langle x_i, a \rangle +  \frac{t}{T} \frac{\d }{\d x_{i}} \langle v_i, a \rangle\\
    = & ~ (1 - \frac{t}{T}) \cdot \frac{\d }{\d x_{i}} \langle x_i, a \rangle\\
    = & ~ (1 - \frac{t}{T}) \cdot a
\end{align*}    
where the first step follows from Definition~\ref{def:z_i}, the second step follows from the Linearity of the Inner Product, the third step follows from Fact~\ref{fac:calculus}, the fourth step follows from variables are independent, and the last step follows from Fact~\ref{fac:calculus}.

\end{proof}

\begin{lemma}\label{lem:gradient_exp_za}
If the following conditions hold
\begin{itemize}
    \item Let $x_i \in \R^d$ for $i=1,2,\dots,n$. 
    \item Let $z_i$ be defined as Definition~\ref{def:z_i}.
    \item Let $a \in \R^d$.
    \item Let $t \in \R$, $T \in \R$, and $0\leq t \leq T$.
\end{itemize}
Then, for each $i \in [n]$, we have
\begin{align*}
    \frac{\d \exp(\langle z_i, a \rangle ) }{ \d x_{i} } = \exp(\langle z_i, a \rangle) (1 - \frac{t}{T}) \cdot a
\end{align*}
\end{lemma}

\begin{proof}
We can show
\begin{align*}
    \frac{\d \exp(\langle z_i, a \rangle ) }{ \d x_{i} } = & ~ \frac{\d \exp(\langle z_i, a \rangle ) }{ \d \langle z_i, a\rangle } \frac{\d \langle z_i, a\rangle}{\d x_{i}}\\
    = & ~ \exp(\langle z_i, a \rangle) \frac{\d \langle z_i, a\rangle}{\d x_{i}}\\
    = & ~ \exp(\langle z_i, a \rangle) (1 - \frac{t}{T}) \cdot a
\end{align*}
where the first step follows from Fact~\ref{fac:calculus}, the second step follows from Fact~\ref{fac:calculus}, and the last step follows from Lemma~\ref{lem:gradient_inner_za}.
\end{proof}

\begin{lemma}\label{lem:gradient_alpha}
    If the following conditions hold
\begin{itemize}
    \item Let $x_i \in \R^d$ for $i=1,2,\dots,n$. 
    \item Let $z_i$ be defined as Definition~\ref{def:z_i}.
    \item Let $\alpha(Z)$ be defined as Definition~\ref{def:alpha}.
    \item Let $Z= [z_1 ~ z_2 ~ \cdots ~ z_n]^\top \in \R^{n \times d}$.
    \item Let $a \in \R^d$.
    \item Let $t \in \R$, $T \in \R$, and $0\leq t \leq T$.
\end{itemize}
Then, for each $i \in [n]$, we have
\begin{align*}
    \frac{\d \alpha(Z)}{\d x_i} = \exp(\langle z_i, a \rangle) (1 - \frac{t}{T}) \cdot a
\end{align*}
\end{lemma}

\begin{proof}
We can show
\begin{align*}
    \frac{ \d \alpha(Z) }{ \d x_{i} } = & ~ \frac{ \d  }{ \d x_{i} } \langle {\bf 1}_n, \exp(Z a) \rangle\\
    = & ~ \frac{ \d  }{ \d x_{i} } \exp(\langle Z, a \rangle)_i\\
    = & ~ \frac{ \d  }{ \d x_{i} }  \exp(\langle z_i, a \rangle)\\
    = & ~ \exp(\langle z_i, a \rangle) (1 - \frac{t}{T}) \cdot a
\end{align*}
where the first step follows from Definition~\ref{def:alpha}, the second step follows from Fact~\ref{fac:calculus}, the third step follows from Fact~\ref{fac:calculus}, and the last step follows from Lemma~\ref{lem:gradient_exp_za}.
\end{proof}

\begin{lemma}\label{lem:gradient_alpha_to_neg_1}
    If the following conditions hold
\begin{itemize}
    \item Let $x_i \in \R^d$ for $i=1,2,\dots,n$. 
    \item Let $z_i$ be defined as Definition~\ref{def:z_i}.
    \item Let $\alpha(Z)$ be defined as Definition~\ref{def:alpha}.
    \item Let $Z= [z_1 ~ z_2 ~ \cdots ~ z_n]^\top \in \R^{n \times d}$.
    \item Let $a \in \R^d$.
    \item Let $t \in \R$, $T \in \R$, and $0\leq t \leq T$.
\end{itemize}
Then, for each $i \in [n]$, we have
\begin{align*}
    \frac{\d \alpha(Z)^{-1}}{\d x_i} = - \alpha(Z)^{-2} \exp(\langle z_i, a \rangle) (1 - \frac{t}{T}) \cdot a
\end{align*}
\end{lemma}

\begin{proof}
\begin{align*}
    \frac{ \d \alpha(Z)^{-1} }{ \d x_{i} } = & ~ \frac{\d \alpha(Z)^{-1}}{\d \alpha(Z)} \frac{\d \alpha(Z)}{\d x_{i}}\\
    = & ~ - \alpha(Z)^{-2} \frac{\d \alpha(Z)}{\d x_{i}}\\
    = & ~ - \alpha(Z)^{-2} \exp(\langle z_i, a \rangle) (1 - \frac{t}{T}) \cdot a
\end{align*}
where the first step follows from Fact~\ref{fac:calculus}, the second step follows from Fact~\ref{fac:calculus}, and the last step follows from Lemma~\ref{lem:gradient_alpha}.
\end{proof}


The score function softmax pmf for discrete case when time considered.

\Yufa{I believe this whole section is not proceeded further and we discussed that the discrete case has problem.}

\begin{lemma}\label{lem:gradient_p_t}
    If the following conditions hold
\begin{itemize}
    \item Let $x_i \in \R^d$ for $i=1,2,\dots,n$. 
    \item Let $z_i$ be defined as Definition~\ref{def:z_i}.
    \item Let $\alpha(Z)$ be defined as Definition~\ref{def:alpha}.
    \item Let $p_t(z_i)$ be defined as Definition~\ref{def:p_t}.
    \item Let $Z= [z_1 ~ z_2 ~ \cdots ~ z_n]^\top \in \R^{n \times d}$.
    \item Let $a \in \R^d$.
    \item Let $t \in \R$, $T \in \R$, and $0\leq t \leq T$.
\end{itemize}
Then, for each $i \in [n]$, we have
\begin{align*}
    \frac{\d p_t(z_i)}{\d x_i} = (- (p_t(z_i))^2 + p_t(z_i))(1 - \frac{t}{T}) \cdot a
\end{align*}
\end{lemma}

\begin{proof}
We can show
\begin{align*}
    \frac{\d p_t(z_i)}{\d x_i} = & ~ \frac{\d }{\d x_i} ( \alpha(Z)^{-1} \exp(\langle z_i, a\rangle) ) \\
    = & ~ (\frac{\d}{\d x_{i}} \alpha(Z)^{-1}) \exp(\langle z_i, a\rangle) + \alpha(Z)^{-1}\frac{\d}{\d x_{i}} \exp(\langle z_i, a\rangle)\\
    = & ~ (- \alpha(Z)^{-2} \exp(\langle z_i, a \rangle) (1 - \frac{t}{T}) \cdot a) \exp(\langle z_i, a\rangle)  + \alpha(Z)^{-1}\frac{\d}{\d x_{i}} \exp(\langle z_i, a\rangle)\\
    = & ~ (- \alpha(Z)^{-2} \exp(\langle z_i, a \rangle) (1 - \frac{t}{T}) \cdot a)\exp(\langle z_i, a\rangle)  + \alpha(Z)^{-1} \exp(\langle z_i, a \rangle) (1 - \frac{t}{T}) \cdot a\\
    = & ~ - (p_t(z_i))^2 (1 - \frac{t}{T}) \cdot a + p_t(z_i) (1 - \frac{t}{T}) \cdot a\\
    = & ~ (- (p_t(z_i))^2 + p_t(z_i))(1 - \frac{t}{T}) \cdot a
\end{align*}
where the first step follows from Definition~\ref{def:p_t}, the second step follows from Fact~\ref{fac:calculus}, the third step follows from Lemma~\ref{lem:gradient_alpha_to_neg_1}, the fourth step follows from Lemma~\ref{lem:gradient_exp_za}, the fifth step follows from Definition~\ref{def:p_t}, and the last step follows from rearranging terms.
\end{proof}

\subsection{Calculation of the score function}


\begin{lemma}\label{lem:gradient_log_p_t}
If the following conditions hold
\begin{itemize}
    \item Let $x_i \in \R^d$ for $i=1,2,\dots,n$. 
    \item Let $z_i$ be defined as Definition~\ref{def:z_i}.
    \item Let $p_t(z_i)$ be defined as Definition~\ref{def:p_t}.
    \item Let $a \in \R^d$.
    \item Let $t \in \R$, $T \in \R$, and $0\leq t \leq T$.
\end{itemize}
Then, for each $i \in [n]$, we have
\begin{align*}
    \frac{\d \log p_t(z_i)}{\d x_i} = (1-p_t(z_i)) (1 - \frac{t}{T}) \cdot a
\end{align*}
\end{lemma}

\begin{proof}
We can show
\begin{align*}
    \frac{\d \log p_t(z_i)}{\d x_i} = & ~ \frac{\d \log p_t(z_i)}{\d p_t(z_i)} \frac{\d p_t(z_i)}{\d x_i}\\
    = & ~ \frac{1}{p_t(z_i)} \frac{\d p_t(z_i)}{\d x_i}\\
    = & ~ \frac{1}{p_t(z_i)} (- (p_t(z_i))^2 + p_t(z_i))(1 - \frac{t}{T}) \cdot a \\
    = & ~ (1-p_t(z_i)) (1 - \frac{t}{T}) \cdot a
\end{align*}
where the first step follows from Fact~\ref{fac:calculus}, the second step follows from Fact~\ref{fac:calculus}, the third step follows from Lemma~\ref{lem:gradient_p_t}, and the last step follows from rearranging terms.
\end{proof}

\subsection{Upper bound for the score function}

\begin{lemma}[Linear growth]
If the following conditions hold
\begin{itemize}
    \item Let $x_i \in \R^d$ for $i=1,2,\dots,n$. 
    \item Let $z_i$ be defined as Definition~\ref{def:z_i}.
    \item Let $p_t(z_i)$ be defined as Definition~\ref{def:p_t}.
    \item Let $a \in \R^d$.
    \item Let $t \in \R$, $T \in \R$, and $0\leq t \leq T$.
\end{itemize}
Then, for $i \in [n]$, we have
\begin{align*}
    \|\frac{\d \log p_t(z_i)}{\d x_i}\|_2 \leq (1 - \frac{t}{T}) \| a \|_2
\end{align*}
\end{lemma}

\begin{proof}
We can show
\begin{align*}
    \|\frac{\d \log p_t(z_i)}{\d x_i}\|_2 = & ~ \|(1-p_t(z_i)) (1 - \frac{t}{T}) \cdot a\|_2\\
    = & ~ (1-p_t(z_i)) (1 - \frac{t}{T}) \cdot \|a\|_2\\
    \leq & ~ (1 - \frac{t}{T}) \cdot \| a \|_2
\end{align*}
where the first step follows from Lemma~\ref{lem:gradient_log_p_t}, the second step follows from Fact~\ref{fac:norm_bounds}, and the last step follows from $0\leq p_t(z_i)\leq 1$.
\end{proof}


\subsection{Lipschitz calculation for the score function}

\begin{lemma}
If the following conditions hold
\begin{itemize}
    \item Let $x_i \in \R^d$ for $i=1,2,\dots,n$. 
    \item Let $z_i$ be defined as Definition~\ref{def:z_i}.
    \item Let $p_t(z_i)$ be defined as Definition~\ref{def:p_t}.
    \item Let $a \in \R^d$.
    \item Let $t \in \R$, $T \in \R$, and $0\leq t \leq T$.
    \item Let $z_i = (1 - \frac{t}{T}) x_i+ \frac{t}{T} v_i$
    \item Let $\wt{z}_i = (1 - \frac{t}{T}) \wt{x}_i +\frac{t}{T} \wt{v}_i$
    \item Let $\alpha(Z)$ be defined as Definition~\ref{def:alpha}.
    \item Let $Z= [z_1 ~ z_2 ~ \cdots ~ z_n]^\top \in \R^{n \times d}$.
    \item Let $\wt{Z}= [\wt{z}_1 ~ \wt{z}_2 ~ \cdots ~ \wt{z}_n]^\top \in \R^{n \times d}$.
\end{itemize}
Then, for $i \in [n]$, we have
\begin{align*}
   | (p_t(z_i)-p_t( \wt{z}_i)) | \leq
\end{align*}
\end{lemma}

\begin{proof}
We can show
\begin{align*}
    | (p_t(z_i)-p_t( \wt{z}_i)) | = & ~ |\alpha(Z)^{-1} \exp(\langle z_i, a\rangle) - \alpha(\wt{Z})^{-1} \exp(\langle \wt{z}_i, a\rangle)|\\
    \leq & ~ |\alpha(Z)^{-1} \exp(\langle z_i, a\rangle) - \alpha(Z)^{-1} \exp(\langle \wt{z}_i, a\rangle)| + |\alpha(Z)^{-1} \exp(\langle \wt{z}_i, a\rangle)- \alpha(\wt{Z})^{-1} \exp(\langle \wt{z}_i, a\rangle)|\\
    = & ~ |\alpha(Z)^{-1} (\exp(\langle z_i, a\rangle) - \exp(\langle \wt{z}_i, a\rangle))| + |(\alpha(Z)^{-1} - \alpha(\wt{Z})^{-1} )\exp(\langle \wt{z}_i, a\rangle)| \\ 
\end{align*}
\Yufa{We discussed for this part and not proceed further.}
\end{proof}




\begin{lemma}[Lipschitz]
If the following conditions hold
\begin{itemize}
    \item Let $x_i \in \R^d$ for $i=1,2,\dots,n$. 
    \item Let $z_i$ be defined as Definition~\ref{def:z_i}.
    \item Let $p_t(z_i)$ be defined as Definition~\ref{def:p_t}.
    \item Let $a \in \R^d$.
    \item Let $t \in \R$, $T \in \R$, and $0\leq t \leq T$.
    \item Let $z_i = (1 - \frac{t}{T}) x_i+ \frac{t}{T} v_i$
    \item Let $\wt{z}_i = (1 - \frac{t}{T}) \wt{x}_i +\frac{t}{T} \wt{v}_i$
\end{itemize}
Then, for $i \in [n]$, we have
\begin{align*}
   \| \frac{\d \log p_t(z_i)}{\d x_i} - \frac{\d \log p_t( \wt{z}_i )}{\d \wt{x}_i} \|_2 \leq L(t) \cdot \| x_i - \wt{x}_i \|_2
\end{align*}
\end{lemma}

\begin{proof}
We can show
\begin{align*}
   \| \frac{\d \log p_t(z_i)}{\d x_i} - \frac{\d \log p_t(\wt{z}_i)}{\d \wt{x}_i}\|_2 = & ~ \| (1-p_t(z_i)) (1 - \frac{t}{T}) \cdot a - (1-p_t(\wt{z}_i)) (1 - \frac{t}{T}) \cdot a\|_2\\
   = & ~ | (p_t(z_i)-p_t( \wt{z}_i)) | \cdot \| (1 - \frac{t}{T}) \cdot a \|_2\\
   = & ~  | (p_t(z_i)-p_t( \wt{z}_i)) | \cdot (1 - \frac{t}{T}) \| a \|_2\\
   \leq & ~ 
\end{align*}
\Yufa{We discussed for this part and not proceed further.}
\end{proof}

